Cyborg Data: Merging Human with AI Generated Training Data

Automated scoring (AS) systems used in large-scale assessment have traditionally used small statistical models that require a large quantity of hand-scored data to make accurate predictions, which can be time-consuming and costly. Generative Large Language Models are trained on many tasks and have shown impressive abilities to generalize to new tasks with little to no data. While these models require substantially more computational power to make predictions, they still require some fine-tuning to meet operational standards. Evidence suggests that these models can exceed human-human levels of agreement even when fine-tuned on small amounts of data. With this in mind, we propose a model distillation pipeline in which a large generative model, a Teacher, teaches a much smaller model, a Student. The Teacher, trained on a small subset of the training data, is used to provide scores on the remaining training data, which is then used to train the Student. We call the resulting dataset "Cyborg Data", as it combines human and machine-scored responses. Our findings show that Student models trained on "Cyborg Data" show performance comparable to training on the entire dataset, while only requiring 10% of the original hand-scored data.

==> Figures/saved_table4.tex <==

\begin{table*}
\centering
\begin{tabular}{c|rrrr | r r r r} \toprule
                                      & \multicolumn{4}{c}{QWK} & \multicolumn{4}{c}{SMD}  \\
    Original/     & \multicolumn{2}{c}{ELECTRA} & \multicolumn{2}{c}{Modern-BERT}  & \multicolumn{2}{c}{ELECTRA} & \multicolumn{2}{c}{Modern-BERT}\\ 
     Synthetic & Orig. & w/Aug. & Orig. & w/Aug. &  Orig. & w/Aug. & Orig. & w/Aug. \\  \midrule
      10\%/90\% &  0.658  & 0.809 & 0.799 & 0.817 & -0.079 & -0.078 & 0.081  & 0.165 \\
      20\%/80\% &  0.788  & 0.811 & 0.820 & 0.822 & -0.076 & -0.070 & 0.017  & 0.174\\
      30\%/70\% &  0.800  & 0.817 & 0.831 & 0.837 & -0.110 & -0.115 & 0.019  & 0.092\\
      40\%/60\% &  0.804  & 0.817 & 0.838 & 0.839 & -0.132 & -0.113 & 0.008  & 0.065\\
      50\%/50\% &  0.813  & 0.826 & 0.840 & 0.842 & -0.111 & -0.113 & -0.004 & 0.039\\
      60\%/40\% &  0.812  & 0.823 & 0.842 & 0.843 & -0.139 & -0.132 & -0.011 & 0.037\\
      70\%/30\% &  0.814  & 0.825 & 0.842 & 0.843 & -0.176 & -0.113 & -0.008 & 0.024\\
      80\%/20\% &  0.819  & 0.823 & 0.843 & 0.844 & -0.139 & -0.149 & -0.016 & 0.009\\
      90\%/10\% &  0.819  & 0.826 & 0.844 & 0.844 & -0.176 & -0.144 & -0.016 & 0.002\\
   
      \hdashline

     100\%/0\% & 0.813 & -  & 0.844  & - & - & - & - & -  \\ \bottomrule
   
    % & - & - & -  & - \\
    % & - & - & -  & - \\
\end{tabular}
\vspace{.3cm}
 \caption{Average QWKs across five experiments for holistic score prediction using varying numbers of original and augmented training data.}\label{results_lcp}
%  {\label{tab:table-name}target words are in bold.}
\end{table*}

